Lighting, Reflectance and Geometry Estimation from 360$^{\circ}$ Panoramic Stereo

We propose a method for estimating high-definition spatially-varying lighting, reflectance, and geometry of a scene from 360$^{\circ}$ stereo images. Our model takes advantage of the 360$^{\circ}$ input to observe the entire scene with geometric detail, then jointly estimates the scene's properties with physical constraints. We first reconstruct a near-field environment light for predicting the lighting at any 3D location within the scene. Then we present a deep learning model that leverages the stereo information to infer the reflectance and surface normal. Lastly, we incorporate the physical constraints between lighting and geometry to refine the reflectance of the scene. Both quantitative and qualitative experiments show that our method, benefiting from the 360$^{\circ}$ observation of the scene, outperforms prior state-of-the-art methods and enables more augmented reality applications such as mirror-objects insertion.

==> Junxuan CVPR21_ Lighting, Reflectance and Geometry Estimation from 360° Cameras (1)/tables/RN_net.tex <==
\begin{table*}
\centering
{\small

\begin{tabular}{c|c|c}
\hline
\multicolumn{3}{c}{\textbf{Encoder}} \\
\hline
0 &	$7 \times 7$  conv, $k_0$ features , stride 2 &	$H/2 \times W/2 \times k_0$\\
\hline
& $3 \times 3$ max pooling,  stride 2	& $H/4 \times W/4 \times k_0$ \\

   &  ($3 \times 3$ conv, $k_1$ features) $\times 2$, residual	 &$H/4 \times W/4 \times k_1$\\

1&	($3 \times 3$ conv, $k_1$ features) $\times 2$, residual	&$H/4 \times W/4 \times k_1$\\
\hline
&($3 \times 3$ conv, $k_2$ features) $\times 2$, stride 2, residual	& $H/8 \times W/8 \times k_2$\\

2&	($3 \times 3$ conv, $k_2$ features) $\times 2$, residual	&$H/8 \times W/8 \times k_2$\\
\hline
	&($3 \times 3$ conv, $k_3$ features) $\times 2$, stride 2, residual	& $H/16 \times W/16 \times k_3$\\

3	&($3 \times 3$ conv, $k_3$ features) $\times 2$, residual	&$H/16 \times W/16 \times k_3$\\
\hline
	&($3 \times 3$ conv, $k_4$ features) $\times 2$, stride 2, residual	&$H/32 \times W/32 \times k_4$\\

4	&($3 \times 3$ conv, $k_4$ features) $\times 2$, residual	&$H/32 \times W/32 \times k_4$\\
\hline
\end{tabular}
}

\vspace{3mm}

{\footnotesize

\begin{tabular}{c|c|c || c|c|c}
\hline
 \multicolumn{1}{c}{} &  \multicolumn{1}{c}{\textbf{Reflectance   Decoder}}  &   \multicolumn{1}{c||}{}  &   \multicolumn{1}{c}{} &   \multicolumn{1}{c}{\textbf{Normal   Decoder }}  &  \multicolumn{1}{c}{} \\
\hline
  &  $2 \times$ bilinear upsample  &  $H/16 \times W/16 \times k_4$  &    &  $2 \times$ bilinear upsample  &  $H/16 \times W/16 \times k_4$\\
  &  ($3 \times 3$ conv, $k_3$ features) $\times 2$, residual  &  $H/16 \times W/16 \times k_3$  &    &    &  \\
$r_1$  &  ($3 \times 3$ conv, $k_3$ features) $\times 2$, residual  &  $H/16 \times W/16 \times k_3$  &  $n_1$  &  ($3 \times 3$ conv, $k_3$ features) $\times 2$, residual  &  $H/16 \times W/16 \times k_3$\\
\hline
&  Add 3 and $r_1$  &  $H/16 \times W/16 \times k_3$  &    &  Add 3 and $n_1$  &  $H/16 \times W/16 \times k_3$\\
  &  $2 \times$ bilinear upsample  &  $H/8 \times W/8 \times k_3$  &    &  $2 \times$ bilinear upsample  &  $H/8 \times W/8 \times k_3$\\
  &  ($3 \times 3$ conv, $k_2$ features) $\times 2$, residual  &  $H/8 \times W/8 \times k_2$  &    &    &  \\
$r_2$  &  ($3 \times 3$ conv, $k_2$ features) $\times 2$, residual  &  $H/8 \times W/8 \times k_2$  &  $n_2$  &  ($3 \times 3$ conv, $k_2$ features) $\times 2$, residual  &  $H/8 \times W/8 \times k_2$\\
\hline
&  Add 2 and $r_2$  &  $H/8 \times W/8 \times k_2$  &    &  Add 2 and $n_2$  &  $H/8 \times W/8 \times k_2$\\
  &  $2 \times$ bilinear upsample  &  $H/4 \times W/4 \times k_2$  &    &  $2 \times$ bilinear upsample  &  $H/4 \times W/4 \times k_2$\\
  &  ($3 \times 3$ conv, $k_1$ features) $\times 2$, residual  &  $H/4 \times W/4 \times k_1$  &    &    &  \\
$r_3$  &  ($3 \times 3$ conv, $k_1$ features) $\times 2$, residual  &  $H/4 \times W/4 \times k_1$  &  $n_3$  &  ($3 \times 3$ conv, $k_1$ features) $\times 2$, residual  &  $H/4 \times W/4 \times k_1$\\
\hline
&  Add 1 and $r_3$  &  $H/4 \times W/4 \times k_1$  &    &  Add 1 and $n_3$  &  $H/4 \times W/4 \times k_1$\\
  &  $2 \times$ bilinear upsample  &  $H/2 \times W/2 \times k_1$  &    &  $2 \times$ bilinear upsample  &  $H/2 \times W/2 \times k_1$\\
  &  ($3 \times 3$ conv, $k_0$ features) $\times 2$, residual  &  $H/2 \times W/2 \times k_0$  &    &    &  \\
$r_4$  &  ($3 \times 3$ conv, $k_0$ features) $\times 2$, residual  &  $H/2 \times W/2 \times k_0$  &  $n_4$  &  ($3 \times 3$ conv, $k_0$ features) $\times 2$, residual  &  $H/2 \times W/2 \times k_0$\\
\hline
&  Add 0 and $r_4$  &  $H/2 \times W/2 \times k_0$  &    &  Add 0 and $n_4$  &  $H/2 \times W/2 \times k_0$\\
  &  $2 \times$ bilinear upsample  &  $H \times W \times k_0$  &    &  $2 \times$ bilinear upsample  &  $H \times W \times k_0$\\
  &  ($3 \times 3$ conv, $k_5$ features) $\times 2$, residual  &  $H \times W \times k_5$  &    &    &  \\
$r_5$  &  ($3 \times 3$ conv, $k_5$ features) $\times 2$, residual  &  $H \times W \times k_5$  &  $n_5$  &  ($3 \times 3$ conv, $k_5$ features) $\times 2$, residual  &  $H \times W \times k_5$\\
\hline
Reflectance  &  $3 \times 3$  conv, 3 features  &  $H \times W \times 3$  &  Normal  &  $3 \times 3$  conv, 3 features  &  $H \times W \times 3$\\
\hline
\end{tabular}
}
\vspace{1mm}
\caption{Network architecture of RN-Net.  All convolutional layers use a ReLu activation and Batch normalization, except for the prediction layer. For RN-Net in original scale $\Phi_{1}$, we set $H=512, W=1024$ and $k_{0,...,5}=[10, 16, 32, 64, 128, 10]$.  For RN-Net in small scale $\Phi_{\frac{1}{4}}$, we set $H=128, W=256$ and $k_{0,...,5}=[64, 64, 128, 256, 512, 32]$.}
\label{tab:rn-net}
\end{table*}

==> Junxuan CVPR21_ Lighting, Reflectance and Geometry Estimation from 360° Cameras (1)/tables/ablation.tex <==
\begin{table}
\centering
{\small
\begin{tabular}{|c|c|c|c|}
\hline
    &  $\Phi_1$   &  $\Phi_{1+\frac{1}{4}}$ & Render and Refine \\
\hline
Reflectance  &   0.086   & 0.080   & \textbf{0.073}       \\
\hline
Normal &  47.3   & \textbf{24.6}  &  -\\
\hline
\end{tabular}
}
\caption{Quantitative results on ablated versions of our model.  We use sMSE for reflectance and MAE for normal.}
\label{tab:ablation}
\end{table}

==> Junxuan CVPR21_ Lighting, Reflectance and Geometry Estimation from 360° Cameras (1)/tables/albedo_normal_others.tex <==
\begin{table}
\centering
{\small
\begin{tabular}{|c|c|c|}
\hline
Methods & Reflectance & Normal \\
\hline
Barron~\etal~\cite{barron2013intrinsic}  &   0.108   & 70.6          \\
\hline
Li~\etal~\cite{li2020inverse}   &  0.084   & 34.0 \\
\hline
Ours   &  \textbf{0.073}   & \textbf{24.6} \\
\hline
\end{tabular}
}
\caption{Quantitative comparison on our synthetic scenes. We use sMSE for reflectance and MAE in degrees for normal.}
\label{tab:albedo_normal}
\end{table}

==> Junxuan CVPR21_ Lighting, Reflectance and Geometry Estimation from 360° Cameras (1)/tables/albedo_normal_others_new.tex <==
\begin{table}
\centering
{\small
\begin{tabular}{|c|c|c|}
\hline
Methods & Reflectance & Normal \\
\hline
Barron~\etal~\cite{barron2013intrinsic}  &   (\sout{0.161})
 0.108   & (\sout{73.9}) 70.6          \\
\hline
Li~\etal~\cite{li2020inverse}   &  0.084   & 34.0 \\
\hline
Ours   &  \textbf{0.073}   & \textbf{24.6} \\
\hline
\end{tabular}
}
\caption{\textbf{Correction of Table 1} in the main paper.
We found an implementation error when testing  Barron~\etal~\cite{barron2013intrinsic} on our data. We are sorry for any  inconvenient. But the new result does not change our analysis and conclusion on the main paper. 
Quantitative comparison on our synthetic scenes is shown in the table. 
We use scale-invariant mean-square-error for reflectance and mean angular error in degrees for normal.  Lower is better for both the metrics.}
\label{tab:albedo_normal}
\end{table}

==> tables/RN_net.tex <==
\begin{table*}
\centering
{\small

\begin{tabular}{c|c|c}
\hline
\multicolumn{3}{c}{\textbf{Encoder}} \\
\hline
0 &	$7 \times 7$  conv, $k_0$ features , stride 2 &	$H/2 \times W/2 \times k_0$\\
\hline
& $3 \times 3$ max pooling,  stride 2	& $H/4 \times W/4 \times k_0$ \\

   &  ($3 \times 3$ conv, $k_1$ features) $\times 2$, residual	 &$H/4 \times W/4 \times k_1$\\

1&	($3 \times 3$ conv, $k_1$ features) $\times 2$, residual	&$H/4 \times W/4 \times k_1$\\
\hline
&($3 \times 3$ conv, $k_2$ features) $\times 2$, stride 2, residual	& $H/8 \times W/8 \times k_2$\\

2&	($3 \times 3$ conv, $k_2$ features) $\times 2$, residual	&$H/8 \times W/8 \times k_2$\\
\hline
	&($3 \times 3$ conv, $k_3$ features) $\times 2$, stride 2, residual	& $H/16 \times W/16 \times k_3$\\

3	&($3 \times 3$ conv, $k_3$ features) $\times 2$, residual	&$H/16 \times W/16 \times k_3$\\
\hline
	&($3 \times 3$ conv, $k_4$ features) $\times 2$, stride 2, residual	&$H/32 \times W/32 \times k_4$\\

4	&($3 \times 3$ conv, $k_4$ features) $\times 2$, residual	&$H/32 \times W/32 \times k_4$\\
\hline
\end{tabular}
}

\vspace{3mm}

{\footnotesize

\begin{tabular}{c|c|c || c|c|c}
\hline
 \multicolumn{1}{c}{} &  \multicolumn{1}{c}{\textbf{Reflectance   Decoder}}  &   \multicolumn{1}{c||}{}  &   \multicolumn{1}{c}{} &   \multicolumn{1}{c}{\textbf{Normal   Decoder }}  &  \multicolumn{1}{c}{} \\
\hline
  &  $2 \times$ bilinear upsample  &  $H/16 \times W/16 \times k_4$  &    &  $2 \times$ bilinear upsample  &  $H/16 \times W/16 \times k_4$\\
  &  ($3 \times 3$ conv, $k_3$ features) $\times 2$, residual  &  $H/16 \times W/16 \times k_3$  &    &    &  \\
$r_1$  &  ($3 \times 3$ conv, $k_3$ features) $\times 2$, residual  &  $H/16 \times W/16 \times k_3$  &  $n_1$  &  ($3 \times 3$ conv, $k_3$ features) $\times 2$, residual  &  $H/16 \times W/16 \times k_3$\\
\hline
&  Add 3 and $r_1$  &  $H/16 \times W/16 \times k_3$  &    &  Add 3 and $n_1$  &  $H/16 \times W/16 \times k_3$\\
  &  $2 \times$ bilinear upsample  &  $H/8 \times W/8 \times k_3$  &    &  $2 \times$ bilinear upsample  &  $H/8 \times W/8 \times k_3$\\
  &  ($3 \times 3$ conv, $k_2$ features) $\times 2$, residual  &  $H/8 \times W/8 \times k_2$  &    &    &  \\
$r_2$  &  ($3 \times 3$ conv, $k_2$ features) $\times 2$, residual  &  $H/8 \times W/8 \times k_2$  &  $n_2$  &  ($3 \times 3$ conv, $k_2$ features) $\times 2$, residual  &  $H/8 \times W/8 \times k_2$\\
\hline
&  Add 2 and $r_2$  &  $H/8 \times W/8 \times k_2$  &    &  Add 2 and $n_2$  &  $H/8 \times W/8 \times k_2$\\
  &  $2 \times$ bilinear upsample  &  $H/4 \times W/4 \times k_2$  &    &  $2 \times$ bilinear upsample  &  $H/4 \times W/4 \times k_2$\\
  &  ($3 \times 3$ conv, $k_1$ features) $\times 2$, residual  &  $H/4 \times W/4 \times k_1$  &    &    &  \\
$r_3$  &  ($3 \times 3$ conv, $k_1$ features) $\times 2$, residual  &  $H/4 \times W/4 \times k_1$  &  $n_3$  &  ($3 \times 3$ conv, $k_1$ features) $\times 2$, residual  &  $H/4 \times W/4 \times k_1$\\
\hline
&  Add 1 and $r_3$  &  $H/4 \times W/4 \times k_1$  &    &  Add 1 and $n_3$  &  $H/4 \times W/4 \times k_1$\\
  &  $2 \times$ bilinear upsample  &  $H/2 \times W/2 \times k_1$  &    &  $2 \times$ bilinear upsample  &  $H/2 \times W/2 \times k_1$\\
  &  ($3 \times 3$ conv, $k_0$ features) $\times 2$, residual  &  $H/2 \times W/2 \times k_0$  &    &    &  \\
$r_4$  &  ($3 \times 3$ conv, $k_0$ features) $\times 2$, residual  &  $H/2 \times W/2 \times k_0$  &  $n_4$  &  ($3 \times 3$ conv, $k_0$ features) $\times 2$, residual  &  $H/2 \times W/2 \times k_0$\\
\hline
&  Add 0 and $r_4$  &  $H/2 \times W/2 \times k_0$  &    &  Add 0 and $n_4$  &  $H/2 \times W/2 \times k_0$\\
  &  $2 \times$ bilinear upsample  &  $H \times W \times k_0$  &    &  $2 \times$ bilinear upsample  &  $H \times W \times k_0$\\
  &  ($3 \times 3$ conv, $k_5$ features) $\times 2$, residual  &  $H \times W \times k_5$  &    &    &  \\
$r_5$  &  ($3 \times 3$ conv, $k_5$ features) $\times 2$, residual  &  $H \times W \times k_5$  &  $n_5$  &  ($3 \times 3$ conv, $k_5$ features) $\times 2$, residual  &  $H \times W \times k_5$\\
\hline
Reflectance  &  $3 \times 3$  conv, 3 features  &  $H \times W \times 3$  &  Normal  &  $3 \times 3$  conv, 3 features  &  $H \times W \times 3$\\
\hline
\end{tabular}
}
\vspace{1mm}
\caption{Network architecture of RN-Net.  All convolutional layers use a ReLu activation and Batch normalization, except for the prediction layer. For RN-Net in original scale $\Phi_{1}$, we set $H=512, W=1024$ and $k_{0,...,5}=[10, 16, 32, 64, 128, 10]$.  For RN-Net in small scale $\Phi_{\frac{1}{4}}$, we set $H=128, W=256$ and $k_{0,...,5}=[64, 64, 128, 256, 512, 32]$.}
\label{tab:rn-net}
\end{table*}

==> tables/albedo_normal_others_new.tex <==
\begin{table}
\centering
{\small
\begin{tabular}{|c|c|c|}
\hline
Methods & Reflectance & Normal \\
\hline
Barron~\etal~\cite{barron2013intrinsic}  &   (\sout{0.161})
 0.108   & (\sout{73.9}) 70.6          \\
\hline
Li~\etal~\cite{li2020inverse}   &  0.084   & 34.0 \\
\hline
Ours   &  \textbf{0.073}   & \textbf{24.6} \\
\hline
\end{tabular}
}
\caption{\textbf{Correction of Table 1} in the main paper.
We found an implementation error when testing  Barron~\etal~\cite{barron2013intrinsic} on our data. We are sorry for any  inconvenient. But the new result does not change our analysis and conclusion on the main paper. 
Quantitative comparison on our synthetic scenes is shown in the table. 
We use scale-invariant mean-square-error for reflectance and mean angular error in degrees for normal.  Lower is better for both the metrics.}
\label{tab:albedo_normal}
\end{table}
